Benchmarking Large Language Models for Molecule Prediction Tasks

Large Language Models (LLMs) stand at the forefront of a number of Natural Language Processing (NLP) tasks. Despite the widespread adoption of LLMs in NLP, much of their potential in broader fields remains largely unexplored, and significant limitations persist in their design and implementation. Notably, LLMs struggle with structured data, such as graphs, and often falter when tasked with answering domain-specific questions requiring deep expertise, such as those in biology and chemistry. In this paper, we explore a fundamental question: Can LLMs effectively handle molecule prediction tasks? Rather than pursuing top-tier performance, our goal is to assess how LLMs can contribute to diverse molecule tasks. We identify several classification and regression prediction tasks across six standard molecule datasets. Subsequently, we carefully design a set of prompts to query LLMs on these tasks and compare their performance with existing Machine Learning (ML) models, which include text-based models and those specifically designed for analysing the geometric structure of molecules. Our investigation reveals several key insights: Firstly, LLMs generally lag behind ML models in achieving competitive performance on molecule tasks, particularly when compared to models adept at capturing the geometric structure of molecules, highlighting the constrained ability of LLMs to comprehend graph data. Secondly, LLMs show promise in enhancing the performance of ML models when used collaboratively. Lastly, we engage in a discourse regarding the challenges and promising avenues to harness LLMs for molecule prediction tasks. The code and models are available at https://github.com/zhiqiangzhongddu/LLMaMol.

==> pages/discussion.tex <==
\textbf{Limitations of LLMs on understanding molecule geometric structure}
A significant limitation of LLMs is their lack of understanding of molecule geometric structure, which in many cases leads to inaccurate results, as shown in Section~\ref{subsec:performance}. 

\smallskip\noindent
\textbf{Flexible framework to incorporate LLMs with existing ML models.}

\smallskip\noindent
\textbf{Molecule specialist LLMs.}
Overall, through an exhaustive set of experiments and analyses, we outline several promising avenues for applying LLMs to molecular prediction tasks. 
While LLMs underperform relative to baselines across a majority of tasks, it’s important to note that LLMs leverage only a few examples to solve chemistry problems, whereas baselines are trained on extensive, task-specific datasets and are limited to certain tasks. 
This observation provides valuable insights into the potential of LLMs’ generalised intelligence in the domain of molecules. 
On the other hand, LLMs display a considerable amount of hallucinations in chemistry tasks, indicating that current LLMs may not yet possess the necessary capabilities to solve practical chemistry problems effectively. 
However, with continuous LLM development and further research into methods to avoid hallucinations, we are optimistic that LLMs can significantly enhance their problem-solving abilities in the field of chemistry.

==> pages/methodology.tex <==
\subsection{Represent Molecules via Text}

\textbf{SMILES String.}

\textbf{Language Description.}
Both structure and attributes are described. 

\subsection{Prompt Engineering}
\label{subsec:prompt_engineering}

\textbf{Input-Feature (\IF)}.
Asking LLMs to extract helpful knowledge for given tasks based on natural language description of the tasks.


==> pages/position_statement.tex <==
TBD
